Enabling Fast and Accurate Crowdsourced Annotation for Elevation-Aware Flood Extent Mapping

Mapping the extent of flood events is a necessary and important aspect of disaster management. In recent years, deep learning methods have evolved as an effective tool to quickly label high resolution imagery and provide necessary flood extent mappings. These methods, though, require large amounts of annotated training data to create models that are accurate and robust to new flooded imagery. In this work, we present FloodTrace, a web-based application that enables effective crowdsourcing of flooded region annotation for machine learning applications. To create this application, we conducted extensive interviews with domain experts to produce a set of formal requirements. Our work brings topological segmentation tools to the web and greatly improves annotation efficiency compared to the state-of-the-art. The user-friendliness of our solution allows researchers to outsource annotations to non-experts and utilize them to produce training data with equal quality to fully expert-labeled data. We conducted a user study to confirm the effectiveness of our application in which 266 graduate students annotated high-resolution aerial imagery from Hurricane Matthew in North Carolina. Experimental results show the efficiency benefits of our application for untrained users, with median annotation time less than half the state-of-the-art annotation method. In addition, using our aggregation and correction framework, flood detection models trained on crowdsourced annotations were able to achieve performance equal to models trained on fully expert-labeled annotations, while requiring a fraction of the time on the part of the expert.

==> Makefile <==
all: paper

CONTENT=compressed-iso-raycasting
BIBLIOGRAPHY=$(wildcard *.bib)
ALLTEXFILES=$(wildcard *.tex content/*.tex)
ALLFIGS=$(wildcard fig/* img/*)
LATEX_ARGS=-halt-on-error -shell-escape

$(CONTENT).pdf: $(ALLTEXFILES) $(ALLFIGS) $(BIBLIOGRAPHY)
	pdflatex $(LATEX_ARGS) $(CONTENT)
	bibtex $(CONTENT)
	pdflatex $(LATEX_ARGS) $(CONTENT)
	pdflatex $(LATEX_ARGS) $(CONTENT)

$(CONTENT)-final.pdf: $(CONTENT).pdf
	gs -sDEVICE=pdfwrite -o $@ \
		-dPDFSETTINGS=/prepress \
		-dDownsampleColorImages=true \
		-dDownsampleGrayImages=true \
		-dDownsampleMonoImages=true \
		-dColorImageResolution=600 \
		-dDoThumbnails=false \
		-f $^

.PHONY: paper
paper: $(CONTENT).pdf

.PHONY: final
final: ${CONTENT}-final.pdf

.PHONY: update_check
update_check:
	mkdir -p ./scripts/
	wget https://raw.githubusercontent.com/erich666/chex_latex/master/chex_latex.pl \
		-O ./scripts/chex_latex.pl

.PHONY: check
check:
	perl ./scripts/chex_latex.pl $(ALLTEXFILES)

.PHONY: clean
clean:
	rm -f *.aux *.bbl *.blg *.dvi *.lbl *.log $(CONTENT).pdf \
		$(CONTENT).out $(CONTENT)-final.pdf *.ps *.brf


==> content/future_work.tex <==
\section{Limitations and Future Work}
\label{sec:future_work} 
%Because efficient use of the semi-automatic tools requires choosing a level of topological simplification, the user needs to experiment first with these settings and switch between simplification levels to be able to select a specific topological feature. As future work, it would be interesting to explore ways to make the selection of simplification levels more friendly to novice users, such as by coupling them to the zoom level in the 3D rendering.
%This is especially true when selecting based on contour tree segmentation, where one can choose too high a simplification level, and then accidentally label features that contain both flooded and dry pixels as one class. One can always select directly on the data with no simplification level though, guaranteeing the selection of a single topological feature of the data but reducing it to its smallest granularity. 
One limitation of our work is that it only supports labeling for two classes of pixels, flooded or dry. Selecting features of the data with more specific labels, such as permanent water bodies, is useful for some flood detection models.
%The mesh creation step (\autoref{sec:rendering}) that we take could also be removed in favor of directly rendering DEM data provided as a heightfield, as described in \cite{kerbltriangle2022, dupuytree2020, cornelheightfield2023}. This would improve the accuracy of our 3D visualization and could enhance user insight into a region. We also find a limitation in the fact that user study participants were more likely to use the brush tools than the elevation-guided tools, and  
There are also limitations with regards to the use of DEM data. As with the machine learning algorithms that rely on DEM data, our system requires that the DEM data and flooded aerial imagery are collected at similar dates. If not, deviations between elevation at the time of flooding and time of DEM collection could lead to annotation error. In addition, it is required that the DEM data precisely matches the region of aerial imagery being annotated, which necessitates careful pre-processing by the researcher. For the study discussed, we downsampled DEM data to match the spatial resolution of the aerial imagery, and have not investigated the effect of using DEM data and aerial imagery with differing resolutions, which could lead to conflict in annotation. Last, the use of DEM data means that objects above the ground level are absent. This is important for labeling areas with tree canopies and buildings, as we wish to consider them flooded if the ground level is flooded. However, for some regions, such as heavily urban environments with many buildings, the presence of these objects could affect water propagation enough to cause the semi-automatic tools to label things incorrectly, for example causing the BFS to falsely label downstream pixels as flooded when the water actually stopped at a building. In the future, it would be interesting to consider semi-automatic tools that utilize digital surface model (DSM) data, taking into account above-ground structures, for use cases on more urban regions.

%The process of using a server backend for topological analysis also comes with drawbacks. Server costs can be prohibitive under substantial traffic, and latency is added between the client submitting their input data and receiving the relevant topological data. In the future, this could help to motivate a Topology Toolkit port to the browser using Javascript, WebAssembly \cite{webassembly}, or WebGPU, or a new library for topological analysis could be built for web development. These seem like good possibilities, as VTK already has a browser library for their functions in VTK.js. This would remove the need for our backend server, and allow all features of our system to take place in the client.

%As it stands, our pipeline for active learning requires manual processing of model predictions, inputting to our application, and then downloading corrected data for retraining. In the future, we see the potential for a full-featured active learning pipeline completely in the browser, where the annotation and visualization frontend communicates directly with the dependent machine learning model. This would allow for immediate user corrections on model predictions, which would automatically retrain the model. By moving the dependent models in the loop of the web-based system, the ability of the user to iterate on steps of prediction, visualization, correction, and retraining would be greatly improved, providing an efficient pipeline for reinforcement learning from human feedback similar to those used by modern language models such as GPT-3.
